GPT-who: An Information Density-based Machine-Generated Text Detector

The Uniform Information Density (UID) principle posits that humans prefer to spread information evenly during language production. We examine if this UID principle can help capture differences between Large Language Models (LLMs)-generated and human-generated texts. We propose GPT-who, the first psycholinguistically-inspired domain-agnostic statistical detector. This detector employs UID-based features to model the unique statistical signature of each LLM and human author for accurate detection. We evaluate our method using 4 large-scale benchmark datasets and find that GPT-who outperforms state-of-the-art detectors (both statistical- & non-statistical) such as GLTR, GPTZero, DetectGPT, OpenAI detector, and ZeroGPT by over $20$% across domains. In addition to better performance, it is computationally inexpensive and utilizes an interpretable representation of text articles. We find that GPT-who can distinguish texts generated by very sophisticated LLMs, even when the overlying text is indiscernible. UID-based measures for all datasets and code are available at https://github.com/saranya-venkatraman/gpt-who.

==> extra_text.tex <==
% \appendix
% \label{sec:appendix}
% \section{Appendix} 
% \subsection{UID Score distribution: ArguGPT dataset}
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\columnwidth]{argugpt_uid.png}
%   \caption{Distribution of UID Scores of 7 models from the ArguGPT dataset.}
% \label{fig:argugpt_uid}
% \end{figure}

% \subsection{UID Score distribution: GPABenchmark}
% \begin{figure}[h!]
% \centering
%     \includegraphics[width=\columnwidth]{gpabench_uid.png}
%   \caption{Distribution of UID Scores of 50k human and 50k GPT generated essays for all 3 writing tasks from the GPABenchmark Dataset across 3 domains \{CS, HSS, PHX\}.}
%   \label{fig:gpabench_uid}
% \end{figure}

% \subsection{UID Score distribution: Deepfake Text Detection in the Wild dataset}
% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=\columnwidth]{testbed2.png}
%    \caption{Distribution of UID Scores of 8 authors (7 models + human) from Deepfake Text Detection in the Wild dataset.}
%     \label{fig:itw_uid5}
% \end{figure}

% \begin{figure}[h!]
%   \begin{subfigure}[b]{\columnwidth}
%          \centering
%         \includegraphics[width=\columnwidth]{testbed1.png}
%          \end{subfigure}
%      \begin{subfigure}[b]{\columnwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{testbed4.png}
%      \end{subfigure}
%     \begin{subfigure}[b]{\columnwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{testbed5.png}
%     \end{subfigure}
%       \begin{subfigure}[b]{\columnwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{testbed1.png}
%     \end{subfigure}
%   \caption{Distribution of UID Scores of human and machine-generated articles corresponding to testbeds from Deepfake Text Detection in the Wild dataset. \label{fig:itw_uid2}}
% \end{figure}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.9\textwidth]{testbed6.png}
%     \caption{UID score distributions of human (h) and model (m) generated texts across 10 domains (indicated by word following either (m\_) or (h\_) along the x-axis) from \citet{li2023deepfake}. Across tasks, humans have a higher mean and wider spread of UID scores than machine-generated text.}
%     \label{fig:itw_uid}
% \end{figure*}


==> tables.tex <==
\begin{table*}[t]
    \centering
    \small
    \renewcommand{\arraystretch}{1.25}
    \begin{tabular}{llccccccc}
        \toprule
        Task Type & Domain & GPTZero & ZeroGPT & OpenAI Detector & DetectGPT & BERT & ITW & {\gptwho} \\
        \midrule

        & CS & 0.30 & 0.67 & 0.81  & 0.58  & \textbf{0.99} & \underline{0.98} & \textbf{0.99} \\
        & PHX & 0.25 & 0.68  & 0.70  & 0.54  &  \textbf{0.99} & \underline{0.98} & \underline{0.98} \\ 
        \multirow{-3}{*}{Task 1} & HSS & 0.72 & 0.92  & 0.63  & 0.57  & \textbf{0.99} & 0.96 & \underline{0.98}\\
        \midrule
         & CS& 0.17  & 0.25  & 0.64 & 0.16 & \textbf{0.99}  & 0.81 & \underline{0.84} \\
         & PHX& 0.06 & 0.10 & 0.24 & 0.17 & \textbf{0.96}& 0.76  & \underline{0.90} \\
        \multirow{-3}{*}{Task 2} & HSS & 0.44   & 0.62 & 0.27& 0.20 & \textbf{0.97}  & 0.29 & \underline{0.80}\\  
        \midrule
         & CS  & 0.02 & 0.03  & 0.06  & 0.03  & \textbf{0.97} & 0.38 & \underline{0.63} \\
         & PHX  & 0.02 & 0.03  & 0.04  & 0.05  & \textbf{0.97} & 0.31  & \underline{0.75}\\
        \multirow{-3}{*}{Task 3} & HSS  & 0.20 & 0.25  & 0.06 & 0.06  & \textbf{0.99}  & 0.08  & \underline{0.62}\\ 
        \midrule
        Average F1 & & 0.24 & 0.40 & 0.38 & 0.26 & \textbf{0.98} & 0.62 & \underline{0.83} \\
        \bottomrule
    \end{tabular}
    \caption{Test Set Performance (F1 Scores) of different machine text detectors on the GPA Benchmark. ITW refers to the LongFormer-based detector trained by \citet{li2023deepfake}. Best performance are in bold, and second best underlined.} 
    \label{tab:gpabench_result}

\bigskip

    \centering
    \begin{tabular}{lcccccc}
        \toprule
        Human v. & GTLR & GPTZero & DetectGPT & BERT & ITW & {\gptwho} \\
        \midrule
        GPT-1 & 0.47 & 0.47 & & \underline{0.95} & 0.92 & \textbf{1.00} \\
        GPT-2\_small & 0.51 & 0.51 & &  \underline{0.75} & 0.47 & \textbf{0.88} \\
        GPT-2\_medium & 0.49 & 0.50 & &  \underline{0.65} & 0.47 & \textbf{0.87} \\
        GPT-2\_large & 0.46 & 0.49 & &  \underline{0.73} & 0.46 & \textbf{0.88} \\
        GPT-2\_xl & 0.45 & 0.51 & &  \underline{0.79 }& 0.45 & \textbf{0.89} \\
        GPT-2\_PyTorch & 0.72 & 0.50 & & \textbf{0.99} & 0.47 &  \underline{0.85} \\
        GPT-3 & 0.35 & 0.47 & &  \underline{0.79} & 0.48 & \textbf{0.84} \\
        GROVER\_base & 0.39 & 0.52 & & \textbf{0.98} & 0.49 &  \underline{0.81} \\
        GROVER\_large & 0.41 & 0.47 & & \textbf{0.98} & 0.52 &  \underline{0.75} \\
        GROVER\_mega & 0.42 & 0.42 & & \textbf{0.97} & 0.53 &  \underline{0.72} \\
        CTRL & 0.88 & 0.67 & &\textbf{1.00} & 0.91 &  \underline{0.99} \\
        XLM & 0.89 & 0.67 & & \textbf{1.00}& 0.92 &  \underline{0.99} \\
        XLNET\_base & 0.75 & 0.51 & & \textbf{0.99} & 0.84 &  \underline{0.98} \\
        XLNET\_large & 0.88 & 0.67 & & \textbf{1.00} &  \underline{0.93} & \textbf{1.00} \\
        FAIR\_wmt19 & 0.56 & 0.56 & & \textbf{0.93} & 0.49 &  \underline{0.74} \\
        Fair\_wmt20 & 0.49 &  \underline{0.50} & & 0.47 & 0.47 &\textbf{1.00} \\
        TRANSFORMER\_XL & 0.35 & 0.49 & & \textbf{0.97} &  \underline{0.81} & 0.79 \\
        PPLM\_distil & 0.64 & 0.52 & &  \underline{0.88} & 0.51 & \textbf{0.95} \\
        PPLM\_gpt2 &  \underline{0.68} & 0.51 & &\textbf{0.89} & 0.49 & \textbf{0.89} \\
        \midrule
        Average F1 & 0.57 & 0.52 & & \textbf{0.88} &  \underline{0.61} & \textbf{0.88} \\
        \bottomrule
    \end{tabular}
    \caption{Test Set Performance (F1 score) for TuringBench dataset. Overall, {\gptwho} outperforms both statistical and supervised detectors, and is at part with BERT. ITW refers to the LongFormer-based detector trained by Li et al. (2023). }
    \label{tab:turing_bench_result}

\bigskip

     \centering
    \begin{tabular}{llcccccc}
        \toprule
        Detection Setting & Testbed Type & GPTZero & GLTR & DetectGPT & BERT & ITW & {\gptwho} \\
        \midrule
        % \multicolumn{}{c}{In-distribution Detection} \\
        \multirow{4}{*}{In-distribution} & Domain-specific Model-specific & 0.65 & 0.94 & 0.92 & \textbf{0.98} & \underline{0.97} & 0.93 \\
         & Cross-domains Model-specific & 0.63 & 0.84 & 0.6 & \textbf{0.98} & \underline{0.97} & 0.88 \\
        & Domain-specific Cross-models & 0.57 & 0.8 & 0.57 & 0.49 & \textbf{0.87} & \underline{0.86} \\
        & Cross-domains Cross-models & 0.57 & 0.74 & 0.57 & 0.49 & \underline{0.78} & \textbf{0.86} \\
        \midrule
        % \multicolumn{7}{c}{Out-of-distribution Detection} \\
        \multirow{2}{*}{Out-of-distribution}& Unseen Models & 0.58 & 0.65 & 0.6 & \textbf{0.84} & \underline{0.79} & 0.74 \\
        &Unseen Domains & 0.57 & 0.73 & 0.57 & 0.68 & \textbf{0.8} & \underline{0.77} \\
        \midrule
        & Average F1 & 0.60 & 0.78 & 0.64 & 0.74 & \textbf{0.86} & \underline{0.84} \\
        \bottomrule
    \end{tabular}
    \caption{Test Set Performance (F1 score) for InTheWild dataset. ITW refers to the LongFormer-based detector trained by Li et al. (2023) specifically for this benchmark.}
    \label{tab:itw_result}
\end{table*}


